PIFu: Pixel-Aligned Implicit Function for High-Resolution Clothed Human Digitization

We introduce Pixel-aligned Implicit Function (PIFu), a highly effective implicit representation that locally aligns pixels of 2D images with the global context of their corresponding 3D object. Using PIFu, we propose an end-to-end deep learning method for digitizing highly detailed clothed humans that can infer both 3D surface and texture from a single image, and optionally, multiple input images. Highly intricate shapes, such as hairstyles, clothing, as well as their variations and deformations can be digitized in a unified way. Compared to existing representations used for 3D deep learning, PIFu can produce high-resolution surfaces including largely unseen regions such as the back of a person. In particular, it is memory efficient unlike the voxel representation, can handle arbitrary topology, and the resulting surface is spatially aligned with the input image. Furthermore, while previous techniques are designed to process either a single image or multiple views, PIFu extends naturally to arbitrary number of views. We demonstrate high-resolution and robust reconstructions on real world images from the DeepFashion dataset, which contains a variety of challenging clothing types. Our method achieves state-of-the-art performance on a public benchmark and outperforms the prior work for clothed human digitization from a single image.

==> ablation_network.tex <==
\begin{table}[t]
\resizebox{\columnwidth}{!}{
\begin{tabular}{llll|lll}
\hline
        & \multicolumn{3}{l|}{RenderPeople} & \multicolumn{3}{l}{Buff} \\
Methods & Normal     & P2S     & Chamfer    & Normal  & P2S         & Chamfer \\ \hline
vgg16     & 0.125      & 3.02    & 2.25      & 0.144   & 4.65        & 3.08    \\
resnet34    & 0.097      & \textbf{1.49}    & \textbf{1.43}       & 0.099   & 1.68        & 1.50    \\
Ours    & \textbf{0.084}      & 1.52    & 1.50   & \textbf{0.092}   & \textbf{1.15}        & \textbf{1.14} \\ \hline
\end{tabular}
}
\caption{\textbf{Ablation study on the sampling strategy.}}
\label{tab:ablation}
\end{table}
